Over-Reasoning and Redundant Calculation of Large Language Models

Large language models (LLMs) can solve problems step-by-step. While this chain-of-thought (CoT) reasoning boosts LLMs' performance, it is unclear if LLMs \textit{know} when to use CoT and whether those CoT are always necessary to answer the question. This paper shows that LLMs tend to generate redundant calculations and reasoning on a manually constructed math QA dataset, GSM8K-Zero. GSM8K-Zero is constructed such that the questions can be answered without any calculations, but LLMs, including Llama-2 models and Claude-2, tend to generate lengthy and unnecessary calculations to answer the questions. We also conduct experiments to explain why LLMs generate redundant calculations and reasonings. GSM8K-Zero is publicly available at https://github.com/d223302/Over-Reasoning-of-LLMs and https://huggingface.co/datasets/dcml0714/GSM8K-Zero.

==> images/illustration <==
<mxfile host="app.diagrams.net" modified="2023-10-17T07:36:03.612Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/115.0.0.0 Safari/537.36" etag="5FmMGTywA5X5lX_6bC25" version="22.0.4" type="device">
  <diagram id="bhxIrrEK157jgLTk5pUk" name="Page-1">
    <mxGraphModel dx="1434" dy="702" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="827" pageHeight="1169" math="0" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="iKyPpODRRuV4LbWUB5zG-7" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="12.5" y="12" width="340" height="90" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-3" value="&lt;div style=&quot;text-align: justify ; font-size: 10px&quot;&gt;&lt;font face=&quot;Roboto&quot; data-font-src=&quot;https://fonts.googleapis.com/css?family=Roboto&quot; style=&quot;font-size: 10px&quot;&gt;&lt;font style=&quot;font-size: 10px&quot; data-font-src=&quot;https://fonts.googleapis.com/css?family=Roboto&quot;&gt;&lt;span style=&quot;background-color: rgb(212 , 225 , 245)&quot;&gt;A deep-sea monster rises from the waters once every hundred years to feast on a ship and sate its hunger. Over three hundred years, it has consumed 847 people. Ships have been built larger over time, so each new ship has twice as many people as the last ship.&lt;/span&gt;&amp;nbsp;&lt;/font&gt;&lt;span style=&quot;background-color: rgb(255 , 217 , 102)&quot;&gt;How many people were on the ship the monster ate in the first hundred years?&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;" parent="iKyPpODRRuV4LbWUB5zG-7" vertex="1">
          <mxGeometry y="20" width="340" height="70" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-8" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="10" y="122" width="345" height="90" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-1" value="&lt;div style=&quot;text-align: justify ; font-size: 10px&quot;&gt;&lt;font style=&quot;font-size: 10px&quot; face=&quot;Roboto&quot; data-font-src=&quot;https://fonts.googleapis.com/css?family=Roboto&quot;&gt;&lt;span style=&quot;background-color: rgb(212 , 225 , 245)&quot;&gt;A deep-sea monster rises from the waters once every hundred years to feast on a ship and sate its hunger. Over three hundred years, it has consumed &lt;b&gt;&lt;u&gt;847&lt;/u&gt;&lt;/b&gt; people. Ships have been built larger over time, so each new ship has twice as many people as the last ship.&lt;/span&gt; &lt;span style=&quot;background-color: rgb(185 , 224 , 165)&quot;&gt;How many people has it consumed over three hundred years?&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;" parent="iKyPpODRRuV4LbWUB5zG-8" vertex="1">
          <mxGeometry x="2.5" width="340" height="70" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-6" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(b) New Question in GSM8K-Zero&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" parent="1" vertex="1">
          <mxGeometry x="87.5" y="192" width="190" height="20" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-5" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(a) Original Question in GSM8K&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" parent="1" vertex="1">
          <mxGeometry x="92.5" y="102" width="180" height="20" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-19" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="12.5" y="193" width="340" height="180" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-16" value="" style="group" parent="iKyPpODRRuV4LbWUB5zG-19" vertex="1" connectable="0">
          <mxGeometry width="340" height="160" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-4" value="&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font face=&quot;Roboto&quot; style=&quot;font-size: 10px;&quot;&gt;To calculate the total number of people the deep-sea monster has consumed over three hundred years, we can sum up the number of people on each ship the monster has feasted on.&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;&lt;font face=&quot;Roboto&quot; style=&quot;font-size: 10px;&quot;&gt;The first ship had 1 person (since it has been a hundred years), the second ship had 2 people (since the new ship has twice as many people as the last ship), the third ship had 4 people, and so on.&amp;nbsp;&amp;nbsp;&lt;/font&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;(...)&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;The formula is as follows:&amp;nbsp;&lt;/font&gt;&lt;/span&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;S&lt;/span&gt;&lt;sub style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;n&lt;/sub&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt; = a * (r&lt;/span&gt;&lt;sup style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;n&lt;/sup&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt; - 1) / (r - 1)&amp;nbsp;&amp;nbsp;&lt;/span&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;(...)&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;span style=&quot;font-family: roboto;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;Therefore, the deep-sea monster has consumed approximately &lt;font style=&quot;font-size: 10px;&quot; color=&quot;#ea6b66&quot;&gt;&lt;u&gt;&lt;b&gt;2.03 x 10&lt;sup&gt;90&lt;/sup&gt;&lt;/b&gt;&lt;/u&gt; &lt;/font&gt;people over three hundred years.&lt;/font&gt;&lt;/span&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;arcSize=5;" parent="iKyPpODRRuV4LbWUB5zG-16" vertex="1">
          <mxGeometry y="20" width="340" height="140" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-15" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(c) LLM output&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" parent="iKyPpODRRuV4LbWUB5zG-19" vertex="1">
          <mxGeometry x="125" y="160" width="90" height="20" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-54" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="416.5" y="495" width="337.5" height="260" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-55" value="" style="group" parent="iKyPpODRRuV4LbWUB5zG-54" vertex="1" connectable="0">
          <mxGeometry y="-10.336391437308869" width="337.5" height="270.3363914373088" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-56" value="&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;The deep-sea monster consumes ships every 100 years, and over 300 years it would have consumed 3 ships. Given that each new ship has twice as many people as the last ship, it means there&#39;s a series of doubling.&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;Let&#39;s assume the number of people on the first ship is X.\n\nThen the number of people on the second ship (which is twice the first) would be 2X and the number of people on the third ship (twice the second ship) would be 4X.\n\nGiven that the total number of people consumed over three centuries is 847, we can write the equation:&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;X + 2X + 4X = 847\n\nThis simplifies to 7X = 847&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;To find X (the number of people on the first ship), we divide 847 by 7, so X = 121.&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;So, over three hundred years, the Monster has consumed 121 people on the first ship, 242 people on the second ship, and 484 people on the third ship. The total is 847 people.&lt;/font&gt;&lt;br&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;arcSize=5;" parent="iKyPpODRRuV4LbWUB5zG-55" vertex="1">
          <mxGeometry y="26.238532110091743" width="337.5" height="244.0978593272171" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-57" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(b) GPT-4 output&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" parent="1" vertex="1">
          <mxGeometry x="531.5" y="755" width="110" height="30" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-1" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="12.5" y="400" width="345" height="112" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-2" value="&lt;div style=&quot;text-align: justify;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot; face=&quot;Roboto&quot;&gt;&lt;span style=&quot;background-color: rgb(212, 225, 245);&quot;&gt;On a farm, on average every 6 cows produce 108 liters of milk per week. In five weeks the cows produced 2160 liters of milk.&lt;/span&gt; &lt;span style=&quot;background-color: rgb(185, 224, 165);&quot;&gt;How many cows on average produce 108 liters of milk per week on a farm?&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;align=left;" vertex="1" parent="q7HdwlbigbdeCHriL69h-1">
          <mxGeometry x="2.5" y="40" width="340" height="47.11" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-3" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(a) Question in GSM8K-Zero&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" vertex="1" parent="1">
          <mxGeometry x="105" y="490" width="160" height="20" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-4" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="15" y="493" width="340" height="327" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-5" value="" style="group" vertex="1" connectable="0" parent="q7HdwlbigbdeCHriL69h-4">
          <mxGeometry y="-13" width="340" height="340" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-6" value="&lt;div style=&quot;text-align: justify; font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;From the information given, every 6 cows produce 108 liters of milk per week. This means that every week, the number of liters produced by one cow is 108 liters&amp;nbsp;&lt;/font&gt;÷&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;&amp;nbsp;6 cows = 18 liters/cow.&lt;/font&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;In five weeks, the cows produced 2160 liters of milk. On average, this means that 2160 liters / 5 weeks = 432 liters of milk were produced every week.&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot;&gt;&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;If we assume that all the cows produce an equal amount of milk, then the number of cows can be calculated as 432 liters&amp;nbsp;&lt;/font&gt;÷&lt;font style=&quot;font-size: 11px;&quot; face=&quot;Roboto&quot;&gt;&amp;nbsp;18 liters/cow = 24 cows. So, 24 cows on average produce 108 liters of milk per week on a farm.&lt;/font&gt;&lt;/font&gt;&lt;br&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;arcSize=5;" vertex="1" parent="q7HdwlbigbdeCHriL69h-5">
          <mxGeometry y="30" width="340" height="170" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-7" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(b) GPT-4 output&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" vertex="1" parent="q7HdwlbigbdeCHriL69h-5">
          <mxGeometry x="115" y="200" width="110" height="30" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-11" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="414" y="400" width="345" height="112" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-50" value="" style="group" parent="q7HdwlbigbdeCHriL69h-11" vertex="1" connectable="0">
          <mxGeometry width="345" height="112" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-51" value="&lt;div style=&quot;text-align: justify ; font-size: 10px&quot;&gt;&lt;font style=&quot;font-size: 10px&quot; face=&quot;Roboto&quot; data-font-src=&quot;https://fonts.googleapis.com/css?family=Roboto&quot;&gt;&lt;span style=&quot;background-color: rgb(212 , 225 , 245)&quot;&gt;A deep-sea monster rises from the waters once every hundred years to feast on a ship and sate its hunger. Over three hundred years, it has consumed &lt;b&gt;&lt;u&gt;847&lt;/u&gt;&lt;/b&gt; people. Ships have been built larger over time, so each new ship has twice as many people as the last ship.&lt;/span&gt;&lt;/font&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;&amp;nbsp;&lt;/span&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot; ; background-color: rgb(185 , 224 , 165)&quot;&gt;How many people has it consumed over three hundred years?&lt;/span&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;align=left;" parent="iKyPpODRRuV4LbWUB5zG-50" vertex="1">
          <mxGeometry x="2.5" y="20" width="340" height="67.11" as="geometry" />
        </mxCell>
        <mxCell id="iKyPpODRRuV4LbWUB5zG-52" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(a) Question in GSM8K-Zero&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" parent="q7HdwlbigbdeCHriL69h-11" vertex="1">
          <mxGeometry x="92.5" y="89" width="160" height="20" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-12" value="&lt;div style=&quot;text-align: justify ; font-size: 10px&quot;&gt;&lt;font style=&quot;font-size: 10px&quot; face=&quot;Roboto&quot; data-font-src=&quot;https://fonts.googleapis.com/css?family=Roboto&quot;&gt;&lt;span style=&quot;background-color: rgb(212 , 225 , 245)&quot;&gt;A deep-sea monster rises from the waters once every hundred years to feast on a ship and sate its hunger. Over three hundred years, it has consumed &lt;b&gt;&lt;u&gt;847&lt;/u&gt;&lt;/b&gt; people. Ships have been built larger over time, so each new ship has twice as many people as the last ship.&lt;/span&gt;&lt;/font&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;&amp;nbsp;&lt;/span&gt;&lt;strike style=&quot;background-color: rgb(255, 217, 102);&quot;&gt;How many people were on the ship the monster ate in the first hundred years?&lt;/strike&gt;&amp;nbsp;&lt;span style=&quot;background-color: rgb(185, 224, 165); font-family: roboto;&quot;&gt;How many people has it consumed over three hundred years?&lt;/span&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;align=left;" vertex="1" parent="1">
          <mxGeometry x="414" y="100" width="340" height="80" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-13" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(a) Question in GSM8K-Zero&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" vertex="1" parent="1">
          <mxGeometry x="509" y="180" width="160" height="20" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-14" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="22.5" y="203" width="340" height="180" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-17" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(c) LLM output&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" vertex="1" parent="q7HdwlbigbdeCHriL69h-14">
          <mxGeometry x="125" y="160" width="90" height="20" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-15" value="" style="group" vertex="1" connectable="0" parent="1">
          <mxGeometry x="414" y="180" width="340" height="140" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-16" value="&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font face=&quot;Roboto&quot; style=&quot;font-size: 10px;&quot;&gt;To calculate the total number of people the deep-sea monster has consumed over three hundred years, we can sum up the number of people on each ship the monster has feasted on.&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;&lt;font face=&quot;Roboto&quot; style=&quot;font-size: 10px;&quot;&gt;The first ship had 1 person (since it has been a hundred years), the second ship had 2 people (since the new ship has twice as many people as the last ship), the third ship had 4 people, and so on.&amp;nbsp;&amp;nbsp;&lt;/font&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;(...)&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;The formula is as follows:&amp;nbsp;&lt;/font&gt;&lt;/span&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;S&lt;/span&gt;&lt;sub style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;n&lt;/sub&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt; = a * (r&lt;/span&gt;&lt;sup style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;n&lt;/sup&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt; - 1) / (r - 1)&amp;nbsp;&amp;nbsp;&lt;/span&gt;&lt;span style=&quot;font-family: &amp;quot;roboto&amp;quot;&quot;&gt;(...)&lt;/span&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;text-align: justify; font-size: 10px;&quot;&gt;&lt;span style=&quot;font-family: roboto;&quot;&gt;&lt;font style=&quot;font-size: 10px;&quot;&gt;Therefore, the deep-sea monster has consumed approximately &lt;font style=&quot;font-size: 10px;&quot; color=&quot;#ea6b66&quot;&gt;&lt;u&gt;&lt;b&gt;2.03 x 10&lt;sup&gt;90&lt;/sup&gt;&lt;/b&gt;&lt;/u&gt; &lt;/font&gt;people over three hundred years.&lt;/font&gt;&lt;/span&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;spacingLeft=5;spacingRight=5;arcSize=5;" vertex="1" parent="q7HdwlbigbdeCHriL69h-15">
          <mxGeometry y="17.5" width="340" height="122.5" as="geometry" />
        </mxCell>
        <mxCell id="q7HdwlbigbdeCHriL69h-18" value="&lt;b&gt;&lt;font style=&quot;font-size: 12px&quot;&gt;(b) ChatGPT output&lt;/font&gt;&lt;/b&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=11;fontFamily=Roboto;" vertex="1" parent="1">
          <mxGeometry x="519" y="316" width="130" height="30" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>

